Decidable Synthesis of Programs with Uninterpreted Functions

We identify a decidable synthesis problem for a class of programs of unbounded size with conditionals and iteration that work over infinite data domains. The programs in our class use uninterpreted functions and relations, and abide by a restriction called coherence that was recently identified to yield decidable verification. We formulate a powerful grammar-restricted (syntax-guided) synthesis problem for coherent uninterpreted programs, and we show the problem to be decidable, identify its precise complexity, and also study several variants of the problem.

==> recursive-pgm.tex <==
%!TEX root = main.tex

\newcommand{\trcc} {\treeaut{\Aa}_{\text{rcc}}}
\newcommand{\wrcc} {\wordaut{\Aa}_{\text{rcc}}}

\section{Synthesizing Recursive Programs}
\seclabel{recursive-pgm}

We now extend the positive result of~\secref{coherent-synth} to
synthesize coherent, recursive programs that meet user
specifications. The setup for the problem is very similar --- given a
grammar that identifies a class of (now) \emph{recursive} programs,
the goal is to determine if there is a program in the class that is
coherent and correct. In order to do this, we first introduce the
class of recursive programs and their semantics, along with important
notions that will help us outline an algorithmic solution to the
synthesis problem.

\subsection{Recursive Programs and their Semantics}

To keep the presentation simple, we will impose some restrictions on
the program syntax, none of which limit the generality of our
results. Let us fix the set of program variables to be
$V = \set{v_1,v_2,\ldots v_r}$, along with an ordering
$\tuple{V} = v_1, v_2, \ldots v_r$. The programs we consider will have
recursively defined methods, and we fix the names of such methods to
belong to a finite set $M$. We will assume that $m_0 \in M$ denotes
the ``main'' method that is invoked when the program is
executed. Without loss of generality, we will assume that the set of
local variables for any method $m \in M$ is $V$; methods can easily
ignore some variables if they use fewer variables. We will also assume
the set of formal parameters for every method is also $V$, called in
the order $\fixperm{V}$. None of these are serious restrictions. Our
methods will return multiple values back, which are assigned by the
caller to local variables. Therefore, for every method $m$, we fix
$\out{m}$ to be the (ordered) \emph{output variables} of $m$; the
variables in $\out{m}$ will be among the variables in $V$. We require
the output variables in $\out{m}$ to be distinct to avoid implicit
aliasing. Recursive programs are now a sequence of method definitions,
wherein one can call other methods, assign values, use conditional
branching and loops, along with sequencing.
%
\[
\begin{array}{rl}
\pgm_{M,V} ::=& m \poutputs \out{m} \stmt_{M,V} \, \mid \,
\pgm_{M,V} \, \pgm_{M,V}\\

\stmt_{M,V} ::=&
\pskip \,
\mid \, x \passign y \,
\mid \, x \passign f(\vec{z}) \,
\mid \, \passume \, \big(\cond_V\big) \,
\mid \, \passert \, \big(\cond_V\big) \\
&
\mid \, \stmt_{M,V} \, ;\, \stmt_{M,V} \,
\mid \, \pif \, \big(\cond_V\big) \, \pthen \, \stmt_{M,V} \, \pelse \, \stmt_{M,V} \\
&
\mid \, \pwhile \, \big(\cond_V\big) \, \stmt_{M,V} \,
\mid \, \vec{w} \passign m(\fixperm{V}) \\

\cond_V ::=&
x = y \,
\mid \, x \neq y
\end{array}
\]
%
Here $x,y,\vec{z}, \vec{w}$ belong to $V$, and the length of vector
$\vec{w}$ must match the output $\out{m}$. A program is nothing but a
sequence of method definitions, and the main method $m_0$ is invoked
first when the program is run. The new statement in the grammar is
$\vec{w} \passign m(\fixperm{V})$ where a method $m$ is called and
when the call returns, the output values are assigned to the vector
$\vec{w}$ of variables.

Different aspects associated with the semantics of such programs, like
executions, terms, coherence, etc., are sketched informally
below. Precise definitions for many of these concepts were first
presented in~\cite{MMV19}, and for completeness are also given in
\appref{recursive}. Executions of recursive programs are sequences
over the alphabet $\Pi_V$ plus two other collections of symbols ---
$\setpred{\dblqt{\pcall~m}}{m \in M}$ which are events corresponding
to method invocation, and
$\setpred{\dblqt{\vec{z}{\passign}\preturn}}{\vec{z}~in~V}$ which are
events corresponding to a return from a method invocation and the
assignment of outputs to local variables in the caller. The set of
executions of a program can be naturally defined and it forms a
context-free language.

Given a data model that provides an interpretation to the constant and
function symbols, every partial execution naturally maps each program
variable to a value in the universe of the data model; in the
interests of space we skip this definition. The notions of an
execution being feasible in a data model (i.e., all assume statements
must hold when encountered) and a program being correct (i.e., all
executions of the form $\rho\cdot\passert(\pfalse)$ are infeasible in
all data models) can be extended naturally to recursive programs.

Finally, the definition of coherent executions and programs can be
extended to the recursive case. To do this, we need to identify the
syntactic term stored in a variable after a partial execution, the set
of syntactic terms computed during a completed execution, and the
collection of equality assumptions made during an execution. These can
be naturally extended from the non-recursive case using a
call-by-value semantics. Based on these, coherence is defined in
exactly the same manner as in the non-recursive case --- executions
are coherent if they are memoizing and have early assumes, and
programs are coherent if all their executions are coherent. Again, we
skip the formal definition to avoid repetition.

As in the non-recursive case, we will represent recursive programs as
finite trees. Recall that a recursive program is nothing but a
sequence of method definitions. Therefore, our tree representation of
a program will be a binary tree with root labeled $\dblqt{\proot}$,
where the right-most path in the tree will have labels of the form
$\dblqt{m \poutputs \out{m}}$, and the left child of such a node will
be the tree representing the body of the method definition of $m$;
since a method body is nothing but a program statement, we could use a
tree representation very similar to the one used for non-recursive
programs. The formal definition of such trees can be easily worked
out, but is given in \appref{recursive} for completeness.

We conclude this section by recalling the main observations
from~\cite{MMV19} about recursive programs --- that the problems of
determining if a recursive program is coherent, and of determining if
a coherent program is correct are decidable.

% \begin{theorem}[\cite{MMV19}]
% \thmlabel{rec-coherent-verif}
% Given a recursive program $P$, the following problems are decidable in
% $\exptime$.
% \begin{itemize}
% \item Determine if $P$ is coherent.
% \item If $P$ is coherent, determine if $p$ is correct.
% \end{itemize}
\begin{theorem}[\cite{MMV19}]
  \thmlabel{rec-coherent-verif} Given a recursive program $P$,
  checking if $P$ is coherent is decidable in $\exptime$.  Further,
  checking correctness of a coherent recursive program is decidable in
  $\exptime$.
\end{theorem}

The proof of \thmref{rec-coherent-verif} relies on the observation
that there are \emph{visibly pushdown automata}~\cite{Alur2004vpa}
(with respect to the partition of $\Pi_{M,V}$ into call alphabet
$\setpred{\dblqt{\pcall~m}}{m \in M}$, return alphabet
$\setpred{\dblqt{\vec{z}{\passign}\preturn}}{\vec{z}~in~V}$, and
internal alphabet $\Pi_V$)~\footnote{``Visible'' here refers to the
  property that these automata push one symbol on their stack when
  they read $\pcall~m$, pop one symbol on $\vec{z} \passign \preturn$,
  and leave the stack unchanged otherwise.}
$\wordaut{\Aa}_{\text{rcoh}}$ and $\wordaut{\Aa}_{\text{rcor}}$ that
accept the set of all coherent executions, and the set of all coherent
executions that are correct, respectively. Both
$\wordaut{\Aa}_{\text{rcoh}}$ and $\wordaut{\Aa}_{\text{rcor}}$ are of
size $O(2^{\text{poly}(|V|)})$. Since the set of all program
executions is also a visibly context-free language, decidability
follows from taking appropriate automata intersections and checking
for emptiness. By taking automata cross-products, we can conclude
there is a visibly pushdown automaton $\wrcc$ of size
$O(2^{\text{poly}(|V|)})$ accepting the set of all recursive
executions that are both coherent and correct; as in the non-recursive
case, we crucially exploit $\wrcc$ for synthesis.

\subsection{Synthesizing Correct, Coherent Programs}

The approach to synthesizing recursive programs is similar to the
non-recursive case, though more complicated. Once again, given a
grammar $\gram$, the set of trees corresponding to programs generated
by $\gram$ is regular; let $\treeaut{\Aa}_{\gram}$ be the tree
automaton accepting this set of trees. The crux of the proof is to
show that there is a two-way alternating tree automaton $\trcc$ that
accepts exactly the collection of all trees that correspond to
recursive programs that are coherent and correct. The synthesis
algorithm then involves checking if there is a common tree accepted by
both $\treeaut{\Aa}_{\gram}$ and $\trcc$, and if so constructing such
a tree. The latter problem is easily reduced to tree automata
emptiness. Therefore, in the rest of the section, we describe how to
construct the automaton $\trcc$.

The construction of the automaton $\trcc$ is similar to the
construction of $\treeaut{\Aa}_\cohcor$ in the non-recursive case. On
an input tree $t$, $\trcc$ will generate all executions of the program
corresponding to $t$ by walking up and down $t$ and checking if each
one of them is coherent and correct by simulating $\wrcc$. The
challenge is to account for recursive function calls and the fact that
$\wrcc$ is a (visibly) pushdown automaton rather than a simple finite
automaton. Giving a precise formal description of $\trcc$ will be
notationally cumbersome, and will obfuscate the ideas behind the
construction. Therefore, we only outline the informal ideas, and leave
working out the precise details to the reader.

Like in the non-recursive case, $\trcc$ will simulate $\wrcc$ as each
execution is generated. Since $\wrcc$ does not change its stack,
except on $\pcall~m$ and $\vec{z}{\passign}\preturn$, we can simulate
$\wrcc$ on most symbols by simply keeping track of the control state
of $\wrcc$. The interesting case to consider is that of method
invocation. Suppose $\trcc$ is at a leaf labeled
$\dblqt{\vec{z}{\passign}m(\fixperm{V})}$. Let $q$ be the control
state of $\wrcc$ after the execution thus far. Executing the statement
$\vec{z}{\passign}m(\fixperm{V})$ gives a partial trace of the form
$\dblqt{\pcall~m}\cdot\rho\cdot\dblqt{\vec{z}{\passign}\preturn}$,
where $\rho$ is an execution of method $m$. Suppose $\wrcc$ on symbol
$\dblqt{\pcall~m}$ from state $q$ goes to state $q_1$ and pushes
$\gamma$ on the stack. Notice that no matter what $\rho$ (the
execution of method $m$) is, since $\wrcc$ is visibly pushdown, the
stack at the end of $\rho$ will be the same as that at the
beginning. Therefore, $\trcc$ will (nondeterministically) guess the
control state $q_2$ of $\wrcc$ at the end of method $m$. $\trcc$ will
send two copies. One copy will simulate the rest of the program (after
$\vec{z}{\passign}m(\fixperm{V})$) from the state $q'$, which is the
state of $\wrcc$ after reading $\dblqt{\vec{z}{\passign}\preturn}$
from $q_2$ and popping $\gamma$. The second copy will simulate the
method body of $m$ to confirm that there is an execution of $m$ from
state $q_1$ to $q_2$. To simulate the method body of $m$, $\trcc$ will
walk all the way up to the root, and then walk down, until it finds
the place where the definition of $m$ is in the tree. $\trcc$ will
also need to account for the possibility that the call to $m$ does not
terminate; in this case, it will send one copy to simulate the body of
$m$, and if that body ever terminates, $\trcc$ will
reject. \pkcomment{(accept, rather than reject?)} Given this informal
description, one can say that a state of $\trcc$ will be of the form
$(p,q_1,q_2)$, where $q_1$ and $q_2$ are a pair of states of $\wrcc$
with the intuition that $q_1$ is the current state of $\wrcc$, $q_2$
is the target state to reach at the end of the method, and $p$ is some
finite amount of book-keeping information needed to perform tasks like
finding an appropriate method body to simulate, whether the method
will return, etc. Thus, the size of $\trcc$ will be
$O(2^{\text{poly}(|V|)})$.

\begin{theorem}
  \thmlabel{rec-synthesis} The program synthesis problem for
  uninterpreted, coherent, \emph{recursive} programs is decidable in
  $\twoexptime$; in particular the algorithm is doubly exponential in
  the number of program variables and \complexitygrammar~in the size
  of the input grammar. Furthermore, a tree automaton representing the
  set of \emph{all} correct, coherent, recursive programs conforming
  to the grammar can be constructed in the same time.  Finally, the
  program synthesis problem in this case is $\twoexptime$-hard.
\end{theorem}

The $\twoexptime$ lower bound follows from the non-recursive case
(\secref{lower-bound}).

